The Long and the Short of It: The Benefits and Leverage of Ultraviolet-Radio Galaxy Fitting

Traditionally, the far ultraviolet (FUV) to far-infrared (FIR) and radio spectral energy distributions (SEDs) of galaxies have been considered separately despite the common physical process shaping them. In this work, we explore the utility of simultaneously fitting FUV-radio SEDs using an extended version of the ProSpect SED fitting code considering contributions from both free-free and synchrotron emission. We use a small sample of galaxies from the Deep Extragalactic VIsible Legacy Survey (DEVILS) and the Key Insights on Nearby Galaxies: a Far-Infrared Survey with Herschel (KINGFISH) where high-quality and robust FUV-radio data are available to provide an ideal sample for testing a radio extension of ProSpect. As the parameterisation of the radio extension links the radio continuum to the FIR emission, we explore the benefit of using radio continuum measurements as a constraint on the energy balance between dust attenuation and emission. We find that for situations where MIR-FIR photometry is unavailable, including a 1.4 GHz continuum measurement allows for improved accuracy in recovered star formation rates and dust luminosities of galaxies reducing the median uncertainty by 0.1 and 0.2 dex respectively. We also demonstrate that incorporating 3 and 10 GHz measurements allows for further constraint on the energy balance and therefore the star formation rate and dust luminosity. This demonstrates the advantage of extending FUV-FIR SED fitting techniques to radio frequencies, especially as we move into an era where FIR surveys will remain limited and radio data become abundant (i.e. with the SKA and precursors).

==> other.tex <==
Assuming constant inflows and outflows tied to SN (OutflowSN), generating SFHs with roughly the same age and mass but with different SFH shapes results in different gas fractions and therefore metallicities. The faster the SFH ramp up, the closer it gets to a very low gas fraction and therefore a high metallicity - this is reflected in the highest mass bin where SFH ramps up quite quickly and could allow for galaxies to get to low gas fractions and therefore high metallicities (this is generally seen in gas surveys where large quenched ellipticals are undetected). 
Technically these galaxies could then continue to accrete pristine gas (maybe not so much to re-trigger star formation) after they have finished forming stars and the metallicity could then decrease but this isn't detected/measured by ProSpect. 
Reaching a high enough metallicity from quick SF requires a reservoir of gas only marginally more massive than the final stellar mass. Otherwise it can just increase the metallicity quickly without reaching a higher metallicity value. 

Interestingly the lowest mass, lowest metallicity case has plenty of galaxies with quick ramp ups and long decays - suggests that the initial   `burst' of star formation didn't use up a majority of the gas and so the SF could continue and also not reach a particularly high metallicity value

Playing with SFHs to get galaxies at $10^{11}M_\odot$ and with Z=0.05 you need to get to log10(gas fractions) of <-2 to get close. (This is in agreement though with the HI gas fractions from XGASS at these stellar masses - $10^{11}M_\odot$).  
Getting to those kind of gas fractions makes sense at high stellar mass, but far less sense at high stellar mass. 
Also getting to low gas fractions can be done either through only having a limited amount of gas to start with (unlikely) or outflows which preferentially remove low metallicity gas. 


- Counfounding variables? Relationship between SFH, inflows+outflows, metallicity? Do inflows and outflows regulate the SFH or does the SFH impact outflows enough to change the metallicity?  




SPS STUFF

One of the choices required when fitting the SEDs of galaxies is the set of templates, known as stellar population synthesis (SPS) models, used to model the expected emission from stars of certain ages and metallicities.  
The \cite{BruzualStellarpopulationsynthesis2003} SPS model is the most commonly employed SPS model in broad-band SED fitting (see Figure~1 or Table~A1 of \citealt{ThorneDeepExtragalacticVIsible2021} for an outline of the SPS models employed by different SED fitting codes), while the E-MILES SPS models are typically used for full spectral fitting techniques due to the finer wavelength resolution.
However, E-MILES has limited wavelength coverage and does not cover the far ultraviolet for all age templates, and does not cover the near-infrared for the youngest age models (Age $< 450\,$Myr).

The creation of SPS models is conceptually straightforward, but current SPS templates are limited by incomplete isochrone tables, incomplete stellar libraries, and poorly calibrated physics (see \citealt{ConroyModelingPanchromaticSpectral2013} for more details). 
Some of the challenges of SPS models include the potential importance of thermally pulsating asymptotic giant branch stars \citep{MarastonEvidenceTPAGBStars2006}, and the importance of binary evolution \citep{Eldridgeeffectstellarevolution2012,EldridgeBinaryPopulationSpectral2017}. 

As \citet[BC03]{BruzualStellarpopulationsynthesis2003} and \citet[BPASS]{EldridgeBinaryPopulationSpectral2017} are both implemented in \textsc{ProSpect}, we can compare the impact on derived galaxy properties when changing the employed SPS model\footenote{\citet[E-MILES]{VazdekisUVextendedEMILESstellar2016} is also incorporated in \textsc{ProSpect}, but due to the limited wavelength coverage, there are many additional caveats that would make these comparisons far more difficult.}
Using the sample of $\sim7,000$ low redshift ($z<0.06$) GAMA galaxies used in \cite{BellstedtGalaxyMassAssembly2020b, BellstedtGalaxyMassAssembly2021} and the methods described in \cite{BellstedtGalaxyMassAssembly2020b} we re-fit the galaxies using the BPASS. 
The BPASS models include 13 metallicities spanning $Z = 10^{5} - 0.04$, E-MILES has 12 metallicities spanning $Z = 10^{4} - 0.04$, while BC03 only has 5 metallicity templates spanning $Z = 10^{-4} - 0.05$. 
However, BC03 includes a significantly finer sampling of ages with 196 age bins with ages less than 14\,Gyrs while BPASS and E-MILES only have 42 and 52 bins respectively with ages less than 14\,Gyrs. 
BPASS has very high time resolution for young stars ($<100\,$Myrs) with age bins of millions of years, and very coarse resolution for older populations with some bins separated by 3 Gyrs. 
E-MILES on the other hand has more even age resolution with bins separated by 10 million years for young ages, and 500 million years for the oldest populations. 
Note that we do not adapt the fitting process to account for the limited wavelength coverage of the E-MILES templates. 

Figure~\ref{fig:BPASS_BC03_ParameterComparisons} shows comparisons between general galaxy properties derived using BPASS and E-MILES to those derived using BC03. 
The stellar masses show good agreement in both cases, however the stellar masses derived using E-MILES are offset at low stellar masses while those derived using BPASS are offset at high stellar masses. 
In both cases the maximum systematic offset is approximately 0.1\,dex. 
The SFRs show a systematic offset in both cases however the direction of the offset is different between SPS models. 
BPASS recovers systematically lower SFRs at the level of $\sim0.15\,$dex across the entire SFR range. 
E-MILES recovers higher SFRs at a level of $\sim0.1\,$dex however this increases to a $\sim0.3\,$dex offset for the highest star formation rates which could be attributed to its limited wavelength coverage. 

To quantify the ages of galaxies we use the half mass age, which is the time at which the galaxy had formed half of its stellar mass. 
We find that the age recovered in both cases trends similarly with both BPASS and E-MILES recovering older ages for young galaxies, and younger ages for old galaxies.

We also show the difference in recovered metallicity when using E-MILES or BPASS. In both cases, the different choice of SPS model results in significantly different metallicity values than when using BC03. 
The straight line artefacts in both panels are a result of galaxies hitting the upper and lower limits of the metallicity templates.

% This is also shown in Figure~\ref{fig:BPASS_BC03_CSFH} where we show the results from stacking the SFHs derived for each of the galaxies to form the CSFH (as per \citealt{BellstedtGalaxyMassAssembly2020b}). 
% For this comparison we do not include completeness corrections, and as we are incomplete to low-mass, young galaxies we find that the SFRD declines more steeply than literature measurements \citep{MadauCosmicStarFormationHistory2014,GAMA_MAGPHYS,BellstedtGalaxyMassAssembly2020b} over the last 4 billion years. 
% The CSFH derived using BPASS has two prominent bump features at 8 and 10 Gyrs which are unphysical. 
% This is due to the sampling of ages in the BPASS templates, where the 8 and 10\,Gyr templates align perfectly with these features.
% Additionally, the range of \texttt{mperiod} values used when fitting with \textsc{ProSpect} was motivated by the sampling of ages in the BC03 templates which typically do not sample any coarser than 300\,Myrs. 
% This means it is possible for a galaxy's entire SFH to fall in the interpolated range between BPASS age templates. 

% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{Figures/BPASS_BC03_CSFH.png}
%     \caption[Comparison of stacked star formation histories derived using BC03 and BPASS]{Comparison of stacked star formation histories using BC03 (blue) and BPASS (black).
%     For comparison we also show the input data and fit to the CSFH as derived by \citet{MadauCosmicStarFormationHistory2014} in grey and the CSFH derived by \citet{GAMA_MAGPHYS} as the black points. 
%     We also show the forensic CSFH as derived by \citet{BellstedtGalaxyMassAssembly2020b} in orange. 
%     The star formation histories from \citet{BellstedtGalaxyMassAssembly2020b} are derived in the same way as the blue line but includes completeness corrections which have not been applied to this same. }
%     \label{fig:BPASS_BC03_CSFH}
% \end{figure}


Figure~\ref{fig:BPASS_BC03_SFMS} shows the impact of the offset between the BC03, BPASS, and E-MILES fits on the SFMS. 
As BPASS predicts systematically lower SFRs, the SFMS recovered using BPASS is below that recovered using BC03. 
The converse is true for the SFMS recovered using E-MILES, and as a result the SFMS lies above the SFMS derived using the other two SPS models. 
Despite the difference in normalisation, all three SPS models recover the same overall bending trend. 


Figure~\ref{fig:BPASS_BC03_MZR} presents the recovered MZR using BC03, BPASS, and E-MILES. Due to the large offset in metallicities discussed previously, the MZRs recovered using E-MILES and BPASS lie significantly below the MZR recovered using BC03 with the E-MILES MZR falling between the BC03 and BPASS MZRs. 
Despite the offset in metallicity values between the two SPS codes, the derived MZR follow the same trend with low mass galaxies having lower gas metallicities than high mass galaxies. 
The scatter on the MZR relation is highest for the BPASS derived sample however. 



